Modeling Orthographic Variation Improves NLP Performance for Nigerian Pidgin

Nigerian Pidgin is an English-derived contact language and is traditionally an oral language, spoken by approximately 100 million people. No orthographic standard has yet been adopted, and thus the few available Pidgin datasets that exist are characterised by noise in the form of orthographic variations. This contributes to under-performance of models in critical NLP tasks. The current work is the first to describe various types of orthographic variations commonly found in Nigerian Pidgin texts, and model this orthographic variation. The variations identified in the dataset form the basis of a phonetic-theoretic framework for word editing, which is used to generate orthographic variations to augment training data. We test the effect of this data augmentation on two critical NLP tasks: machine translation and sentiment analysis. The proposed variation generation framework augments the training data with new orthographic variants which are relevant for the test set but did not occur in the training set originally. Our results demonstrate the positive effect of augmenting the training data with a combination of real texts from other corpora as well as synthesized orthographic variation, resulting in performance improvements of 2.1 points in sentiment analysis and 1.4 BLEU points in translation to English.

==> sections/4_experiements.tex <==



\section{Experiments}
In this section, we provide the experimental setup for two critical tasks used to test the influence of orthographic variation augmentation: sentiment analysis and machine translation.

\subsection{Datasets and networks}


Table \ref{tab:data} describes the datasets used in our experiments. 
%We employ widely used pre-trained language models for adapting English pre-trained model to two critical tasks: sentiment analysis and machine translation.
For the task of sentiment analysis, we use the NaijaSenti dataset \citep{muhammad-etal-2022-naijasenti}, which comprises a three-way data split (6.7K/0.6K/1.2K) to perform sentiment analysis.
We use ROBERTA and BERT in base versions. We then perform fine-tuning (FT), which directly transfers the pre-trained language model to the Pidgin language. 
All models are evaluated using the F1 score.

For the task of machine translation, we leverage \textsc{T5 Base} for JW300 translation benchmark. The baseline consists of 29K training samples. We perform bi-directional translation for the parallel English-Pidgin datasets, which are the Bible, JW300 \citep{agic2019}, and the Naija Treebank \citep{caron2019surface}. 
All model variants are evaluated on the test set using BLEU score.


%\input{tbls/variation_stat}

\merel{To do Merel: split up into sec5 and 6}

\subsection{Training details}
Following prior work, we used BERT and RoBERTa for sentiment analysis, training the models for 5 epochs with a mini-batch of 32 and report the scores over 6 seeds.
We employed Adam optimization with a learning rate of 0.0001, and we found that a smaller learning rate helped prevent overfitting in the downstream task.

For the machine translation task, we fine-tuned the T5 model with a base size for 20 epochs and a batch size of 16. 
We configured the sequence length to be 196 characters and used the AdamW optimizer \cite{} with a learning rate of 0.0001.

All model variants for both tasks underwent the same number of training epochs as their respective baselines. 
%When appending the orthographic variation data as augmentation, we replaced the original data samples with variation-augmented data samples, each with an optimal K value tailored to its specific task. 
For NaijaSenti, we sample optimal size with K=100. For JW300, we used K=5K, since the training data for the machine translation task is larger. The augmentation samples were drawn from single and various sources, including the Bible, JW300, and Naija Treebank.

\merel{To discuss: pull these apart and include with sec5 and 6?}




% This simple technique has proven to be rather effective, as demonstrated by experimental results (see the following sections), where even a small amount of augmentation yielded significant benefits.

% Several words within a sentence has derived to new generated variations.
% The goal of the variation-augmented data is to improve the generalization of a pre-trained model with potentially noisy samples. 
% As such, the augmented data, denoted as $D'$, comprises both real Pidgin sentences and edited sentences. 
% the sentiment analysis and machine translation tasks by appending new data instances.

% Next, we demonstrate the applications using the generated variations on two crtical tasks.

% In the nature of Pidgin language, the spelling variations originate from common sounds and different speaker, representing distinct domains of data resources and have many possible spellings.

%Orthographic variation augmentation draws inspiration from the concept of \emph{data augmentation}, for which the corpus is augmented with new data instances, often based on real examples.
% Specifically, we introduce \emph{OVa}, which augments the corpus with variation-enhanced sentences as supplementary data.

%\merel{Explain: we take $K$ samples from the existing training dataset, and for these samples we greedily generate a variation for all possible words in a sentence.}


% Variations originate from different sources, representing distinct domains of data resources.
% Concretely, given a new data resource, i.e. ${x_i} \in D$, consist of $M$ data samples.
% We randomly extract the pre-determined $K$ examples from $x_1, ..., x_k$ and replace words with synthesized variations. 
% These $K$ variation-augmented samples are added to the data resource, resulting in $D \cup \{x'_{1}, ,..., x'_{k}\}$.
% %In practice, Mixup Augmentation theoretically considers different data resources. 
% In the next section, we explore the utilization of multiple available data resources, as this approach has the potential to enrich variations across various domains. This simple technique has proven to be rather effective, as demonstrated by experimental results (see the following sections), where even a small amount of augmentation yielded significant benefits.




==> tbls/generalization_treebank.tex <==

\begin{table}[t]
\label{tab:t5}
\centering
% \begin{tabular}{lS[table-format=2.2]S[table-format=2.2]}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lll}
\toprule
\textbf{Model Type} & \textbf{EN.-PG.} & \textbf{PG.-EN.} \\ 
\midrule
% \emph{\textsc{Baseline(TreeBank)}} \\
% \midrule
% DataAug: all real data
\emph{\textsc{w/o orthographic variation}} \\
\textsc{\hspace{3mm}JW300}  & \text{18.06} & \text{13.53} \\
\textsc{\hspace{3mm}JW300+Bible} & \text{8.40} & \text{7.79} \\
% \midrule
% \emph{\textsc{DataAug}} \\
% \textsc{\hspace{3mm}JW300+Bible} & \text{17.43} & \text{17.38} \\
% \textsc{\hspace{3mm}JW300+Bible+TreeBank} & \text{17.45} & \text{17.26} \\ 
\midrule
% MixUp: real + edited data
\emph{\textsc{with orthographic variation}} \\
\textsc{\hspace{3mm}JW300} & \textbf{18.52} & \textbf{13.80} \\
\textsc{\hspace{3mm}JW300+BiBle} & \text{8.61} & \text{8.57} \\
% \textsc{\hspace{3mm}JW300+BiBle+TreeBank} & \textbf{17.67} & \text{17.55} \\
% \midrule
% \emph{\textsc{All}+\textsc{TaT}} \\
% \textsc{\hspace{3mm}T5 (base)} & \textbf{36.35} & \textbf{34.04}  \\ 
\bottomrule
% 36.04 33.99
\end{tabular}}
\caption{ \small \textbf{Results of traditional data augmentation (DataAug) and the proposed argumentation with orthographic variation, generalization on Naija Treebank test set.}}
\end{table}
%  All results on JW300 translation benchmark using \textsc{T5 Base} with \textsc{DataAug} and \textsc{MixupAug}


% old one
% \begin{table}[ht]
% \label{tab:t5}
% \centering
% % \begin{tabular}{lS[table-format=2.2]S[table-format=2.2]}
% \begin{tabular}{lll}
% \toprule
% \textbf{Model Type} & \textbf{En.-PG.} & \textbf{PG.-EN.} \\ 
% \midrule
% \emph{\textsc{JW300, Bible}} \\
% % \textsc{\hspace{3mm}mT5 (\small{small})} & 32.82  & 31.37 \\
% \textsc{\hspace{3mm}mT5 (\small base)} & 33.78 & 32.4  \\ 
% \textsc{\hspace{3mm}T5 (base)} & \textbf{36.16} & \textbf{33.22} \\
% \midrule

% % MixUp
% \XXX{\emph{\textsc{MixUp: JW300, Bible}}} \\
% \textsc{\hspace{3mm}T5 (base)} \\
% \midrule

% \emph{\textsc{JW300, Bible, TreeBank}} \\
% \emph{\textsc{religious,misc.}} \\
% \textsc{\hspace{3mm}mT5 (\small base)} &33.92 & 32.75  \\ 
% \textsc{\hspace{3mm}T5 (base)} & \textbf{36.04} & \textbf{34.02} \\ 
% \midrule


% \emph{\textsc{All}+\textsc{TaT}} \\
% \textsc{\hspace{3mm}T5 (base)} & \textbf{36.35} & \textbf{34.04}  \\ 
% \bottomrule
% % 36.04 33.99
% \end{tabular}
% \caption{ \small \textbf{Results on JW300 translation benchmark using \textsc{T5} and \textsc{mT5}.}}
% \end{table}


==> tbls/number_of_added_variation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[th!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|S[table-format=2.1]S[table-format=2.1]S[table-format=2.1]S[table-format=2.1]}
\toprule
\textbf{MixupAug.} & \textbf{100} & \textbf{1K} & \textbf{3K} & \textbf{\textsc{8K}} \\
\midrule
\textsc{\hspace{3mm}Addition} & \textbf{82.29} & \text{81.23} & \textbf{81.09} & \textbf{81.09} \\ 
\textsc{\hspace{3mm}Replacement} & \text{81.35} & \textbf{81.64} & \text{81.0} & \text{80.1} \\ 
\bottomrule
\end{tabular}}
\caption{\small \textbf{Results of sentiment classification on NaijaSenti (9K).}}

\label{tab:k_size_replacement}
\end{table}



==> tbls/result_on_k_size_replacement.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[th!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|S[table-format=2.1]S[table-format=2.1]S[table-format=2.1]S[table-format=2.1]}
\toprule
\textbf{MixupAug. Strategy} & \textbf{100} & \textbf{1K} & \textbf{3K} & \textbf{\textsc{8K}} \\
\midrule
\textsc{\hspace{3mm}Addition} & \textbf{82.29} & \text{81.23} & \textbf{81.09} & \textbf{81.09} \\ 
\textsc{\hspace{3mm}Replacement} & \text{81.35} & \textbf{81.64} & \text{81.0} & \text{80.1} \\ 
\bottomrule
\end{tabular}}
\caption{\small \textbf{Results of sentiment classification on NaijaSenti.}}
\label{tab:augmentation_strategy}
\end{table}



==> tbls/variation_in_dataset.tex <==

\begin{table}[t]
\small
\centering
\begin{tabular}{l @{\hspace{0.5\tabcolsep}} c @{\hspace{0.1\tabcolsep}} r}
\toprule
{\bfseries Corpus} & {\bfseries $|$Train$|$}& {\bfseries \#variation types} \\
\midrule
\href{https://www.bbc.com/pidgin}{BBC Pidgin}& $4K$ & $188$ \\ %4,147 Pidgin articles
PidginUNMT & $5K$  & $142$ \\
ASR   & $8K$ & $80$ \\
NaijaSenti  & $8.5K$  & $119$ \\
\text{Naija Treebank}   & $9K$ & $51$ \\
\midrule
JW300 & $20K$ & $20$ \\
Bible & $29K$  & $181$ \\
\midrule
Afri-BERTa  & $176K$  & $250$ \\
\bottomrule
\end{tabular}
\caption{\small The variation within the Pidgin corpus. We extract the English word and its varaitions
in each Pidgin text to quantify the degree of variations.
}\label{tab:variation_example}
\end{table}


==> tbls/variation_stat.tex <==

\begin{table}[t]

\centering

\begin{tabular}{l @{\hspace{0.5\tabcolsep}} c @{\hspace{0.1\tabcolsep}} r}
\toprule
{\bfseries Corpus} & {\bfseries $|$Train$|$}& {\bfseries \#variation types} \\
%\midrule
%\multicolumn{3}{c}{\textsc{Parallel}} \\
\midrule

%\midrule
%\multicolumn{3}{c}{\textsc{Monolingual}} \\
%\midrule
\href{https://www.bbc.com/pidgin}{BBC Pidgin}& $4K$ & $188$ \\ %4,147 Pidgin articles
%PidginUNMT & $5K$  & $142$ \\
%ASR   & $8K$ & $80$ \\
NaijaSenti  & $8.5K$  & $119$ \\
\midrule
\text{Naija Treebank}   & $9K$ & $51$ \\
%\midrule
JW300 & $20K$ & $20$ \\
Bible & $29K$  & $181$ \\
%\midrule
%Afri-BERTa  & $176K$  & $250$ \\
\bottomrule
\end{tabular}
\caption{\merel{Footnote? }}\label{tab:variation_count}
\end{table}

